SegMAN: Omni-scale Context Modeling with State Space Models and Local Attention for Semantic Segmentation

High-quality semantic segmentation relies on three key capabilities: global context modeling, local detail encoding, and multi-scale feature extraction. However, recent methods struggle to possess all these capabilities simultaneously. Hence, we aim to empower segmentation networks to simultaneously carry out efficient global context modeling, high-quality local detail encoding, and rich multi-scale feature representation for varying input resolutions. In this paper, we introduce SegMAN, a novel linear-time model comprising a hybrid feature encoder dubbed SegMAN Encoder, and a decoder based on state space models. Specifically, the SegMAN Encoder synergistically integrates sliding local attention with dynamic state space models, enabling highly efficient global context modeling while preserving fine-grained local details. Meanwhile, the MMSCopE module in our decoder enhances multi-scale context feature extraction and adaptively scales with the input resolution. Our SegMAN-B Encoder achieves 85.1% ImageNet-1k accuracy (+1.5% over VMamba-S with fewer parameters). When paired with our decoder, the full SegMAN-B model achieves 52.6% mIoU on ADE20K (+1.6% over SegNeXt-L with 15% fewer GFLOPs), 83.8% mIoU on Cityscapes (+2.1% over SegFormer-B3 with half the GFLOPs), and 1.6% higher mIoU than VWFormer-B3 on COCO-Stuff with lower GFLOPs. Our code is available at https://github.com/yunxiangfu2001/SegMAN.

==> sec/0_abstract.tex <==
\begin{abstract}
% Current state-of-the-art semantic segmentation models cannot effectively model global context, preserve fine-grained local details, and capture multi-scale information simultaneously. To this end, we present LAMSeg, a novel architecture that effectively addresses these challenges through two key innovations: (1) LAMNet, a hybrid encoder that synergistically combines local attention with Mamba, enabling efficient global context modeling while preserving fine-grained spatial details, and (2) MMSCopE, an adaptive decoder that processes full-resolution feature maps with region sizes that scale with input dimensions. Both components achieve linear computational complexity, making them particularly effective for high-resolution inputs. MODELNAME achieves state-of-the-art performance across challenging benchmarks, with our Small variant (29.9M parameters) achieving 50.0\%, 83.1\%, and 46.5\% mIoU on ADE20K, Cityscapes, and COCO-Stuff respectively, while maintaining competitive computational efficiency.

High-quality semantic segmentation relies on three key capabilities: global context modeling, local detail encoding, and multi-scale feature extraction. However, recent methods struggle to possess all these capabilities simultaneously. Hence, we aim to empower segmentation networks to simultaneously carry out efficient global context modeling, high-quality local detail encoding, and rich multi-scale feature representation for varying input resolutions. In this paper, we introduce LAMSeg, a novel linear-time model comprising a hybrid feature encoder dubbed LAMNet, and a decoder based on state space models. Specifically, LAMNet synergistically integrates sliding local attention with dynamic state space models, enabling highly efficient global context modeling while preserving fine-grained local details. Meanwhile, the MMSCopE module in our decoder enhances multi-scale context feature extraction and adaptively scales with the input resolution. We comprehensively evaluate LAMSeg on three challenging datasets: ADE20K, Cityscapes, and COCO-Stuff. For instance, LAMSeg-B achieves 52.1\% mIoU on ADE20K, outperforming SegNeXt-L by 1.1\% mIoU while reducing computational complexity by over 20 GFLOPs. On Cityscapes, LAMSeg-B attains 83.8\% mIoU, surpassing SegFormer-B3 by 2.1\% mIoU with approximately half the GFLOPs. Similarly, LAMSeg-B improves upon VWFormer-B3 by 0.9\% mIoU with lower GFLOPs on COCO-Stuff dataset.

% Notably, LAMSeg-B achieves 52.1\% mIoU with 53 GFLOPs on ADE20K, outperforming previous state-of-the-art by a significant margin.

\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
% This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

As a core computer vision task, semantic segmentation needs to assign a categorical label to every pixel within an image \cite{minaee2021image}. 
% Early breakthroughs emerged through convolutional neural networks (CNNs), such as FCN~\cite{long2015fully}, PSPNet~\cite{zhao2017pyramid} and the DeepLab series~\cite{chen2017deeplab,Chen2017RethinkingAC,chen2018encoder}.
% Recent advances have shifted towards Transformer-based architectures, demonstrating superior performance through both enhanced feature encoders~\cite{xie2021segformer,yu2024edaformer} and specialized decoder heads~\cite{yan2024vwaformer,yu2024edaformer}.
% Despite these advances, the computational demands of dense predictions on high-resolution images (e.g. \(2048\times 1024\) images in Cityscapes) impose challenging constraints to the design of segmentation architectures. Designing network architectures that achieve excellent segmentation performance while maintaining computational efficiency remains a challenging research problem.
% Addressing this problem requires three crucial capabilities that determine segmentation performance. 
Accurate semantic segmentation demands three crucial capabilities. First, \textbf{global context modeling} establishes rich contextual dependencies regardless of spatial distance, enabling overall scene understanding \cite{fu2019dual}. 
Second, \textbf{local detail encoding} learns fine-grained feature and boundary representations, crucial for differentiating semantic categories and localizing boundaries between adjacent regions with different semantic meanings \cite{yu2018learning}.
Third, \textbf{context modeling based on multiple intermediate scales} learns semantic representations across multiple scales, addressing intra-class scale variations while enhancing inter-class discrimination~\cite{zhao2017pyramid,chen2017deeplab,yan2024vwaformer}.
\par
Recent methods for semantic segmentation still do not possess all these three capabilities simultaneously. For instance, VWFormer~\cite{yan2024vwaformer} introduces a varying window attention (VWA) mechanism that effectively captures multi-scale information through cross-attention between local windows and multiple windows with predefined scales. 
However, at higher input resolutions, the global context modeling capability of VWA diminishes because the predefined window sizes fail to maintain full feature map coverage. In addition, larger windows significantly increase the computational cost as self-attention exhibits quadratic complexity. Likewise, EDAFormer~\cite{yu2024edaformer} proposes an embedding-free spatial reduction attention (SRA) mechanism to implement global attention efficiently and an all-attention decoder for global and multi-scale context modeling. 
However, fine-grained details are lost due to its reliance on downsampled features for token-to-region attention.
Moreover, the absence of dedicated local operators in the feature encoder limits fine-grained feature learning~\cite{xie2021segformer,yu2024edaformer}.
\par
%Meanwhile, ViT-CoMer~\cite{xia2024vit} presents a two-branch architecture, comprising a ConvNet for local detail encoding and a pre-trained Vision Transformer (ViT)~\cite{dosovitskiy2020vit} for global context modeling, with multi-scale interaction between the two branches. However, ViT-CoMer has quadratic complexity and does not support interactions between global and local features within the encoder, neglecting many image details and contextual cues.


\begin{figure*}[t]
\centering
    \begin{minipage}[t]{0.34\textwidth}
\centering
\makeatletter\def\@captype{figure}
  \setlength{\abovecaptionskip}{0.1cm}
  \setlength{\belowcaptionskip}{0.2cm}
\includegraphics[width=\textwidth]{sec/Figures/ERF.pdf}
\label{scaling}
\end{minipage}
\quad
\begin{minipage}[t]{0.62\textwidth}
\centering
\makeatletter\def\@captype{figure}
\setlength{\abovecaptionskip}{0.1cm}
\setlength{\belowcaptionskip}{0.2cm}
    \includegraphics[width=\textwidth]{sec/Figures/segmentation_map.pdf}
\label{intro_segmentation_maps}
\end{minipage}
\vspace{-0.4mm}
\caption{Comparison of receptive fields and segmentation quality. \textit{Left}: Visualization of effective receptive fields (ERF) on the Cityscapes validation set at 1024×1024 resolution, illustrating LAMSeg's stronger global context modeling capacity in comparison to existing state-of-the-art models. \textit{Right}: Segmentation maps highlighting LAMSeg's superior capacity to encode fine-grained local details that are often missed by existing approaches.\vspace{-3mm}}
\label{intro_visualization}
\end{figure*}

To present a more intuitive understanding of the aforementioned issues, we visualize the effective receptive field (ERF) maps and segmentation maps of recent state-of-the-art models~\cite{xie2021segformer,yan2024vwaformer,yu2024edaformer}. 
As depicted in Figure~\ref{intro_visualization} (\textit{Left}), the ERF of VWFormer~\cite{yan2024vwaformer} and EDAFormer~\cite{yu2024edaformer} has limited feature map coverage when processing high-resolution Cityscapes images. 
Meanwhile, the segmentation maps in Figure~\ref{intro_visualization} (\textit{Right}) reveal that existing methods have a limited ability to recognize fine-grained local details, which we attribute to insufficient local feature modeling in these architectures.
\par
 % requiring the simultaneous modeling of informative global context with nearly linear complexity, extraction of discriminative and continuous local details, and incorporation of powerful contexts from diverse scales. 
In this work, we aim to encapsulate omni-scale context modeling for a varying input resolution within a semantic segmentation network. As a result, we propose LAMSeg, a novel segmentation network capable of carrying out efficient global context modeling, high-quality local detail encoding, and rich context representation at diverse scales simultaneously. Our LAMSeg introduces two novel sub-networks: a hybrid feature encoder, LAMNet (Local Attentional Mamba Network), and a decoder with a Mamba-based Multi-Scale Context Extraction (MMSCopE) module.
LAMNet features a novel token mixer that integrates a 2D version of state space models (SS2D)~\cite{liu2024vmamba} for global context modeling with neighborhood attention\cite{hassani2023neighborhoodAttn} (Natten) for local detail encoding, both functioning in linear time.
The dynamic global scanning in our method always covers the full feature map, this design enables robust global context modeling across varying input resolutions and all encoder layers. Meanwhile, by performing local attention within a sliding window, Natten exhibits an outstanding capability in fine-grained local detail encoding. On the other hand, leveraging the linear time complexity of Mamba, our decoder complements the encoder with robust feature learning across multiple scales. It first generates multiple versions of an aggregated feature map in different resolutions including the full resolution, each version representing a different scale. Then it employs SS2D to scan these feature maps to learn multi-scale contexts. %This essentially learns context features within adaptive regions that scale with the input resolution.
For higher efficiency, the feature maps at different scales are reshaped to the same resolution and concatenated so that scanning only needs to be performed on a single feature map. 
Note that our method differs from existing methods in two aspects.
First, unlike multi-kernel convolution~\cite{chen2017deeplab} and multi-scale window attention~\cite{yan2024vwaformer}, our design adaptively scales with the input resolution.
Second, by performing SS2D-based scanning over entire multi-scale feature maps, our method better preserves fine-grained details that are typically compromised by pooling operations~\cite{ni2024cgrseg,zhao2017pyramid} or spatial reduction attention~\cite{yu2024edaformer} in existing methods.

% The former is stacked with a novel token mixer comprising VSSM and Neighborhood attention. The motivation behind this design is that, since the feature encoder directly acts on the input image, it should possess the largest possible receptive field to generate a global perception. Hence, we employ VSSM to establish long-range dependencies. Notably, VSSM has linear complexity, differing from global self-attention, and can be used in large resolutions without compressing the input like SRA, thereby acquiring more fine-grained global contexts. Additionally, Neighborhood attention can dynamically model local details in an overlapping approach, generating more powerful local representations. In this regard, our feature encoder can model global contexts at varying input resolutions while preserving strong local inductive biases, which is not achieved in previous segmentation models. Based on the feature encoder, we further propose a simple yet effective Mamba-based decoder that can efficiently model multi-scale contexts based on the pyramid features generated by the feature encoder. Unlike previous works that utilize multi-kernel convolution/pooling layers and multi-scale window attention, which have a fixed range for extracting multi-scale information even when the input resolution increases, our Mamba decoder implements VSSM on aggregated features from different regions, adaptively adjusting according to input resolutions, thereby constructing more robust multi-scale representations under different input resolutions.

Our LAMSeg achieves state-of-the-art performance on three widely used datasets: ADE20K~\cite{zhou2017ade20k}, Cityscapes~\cite{cordts2016cityscapes}, and COCO-Stuff-164k~\cite{caesar2018cocostuff}. 
Notably, our Base variant (53.9M parameters, 52.9 GFLOPs for ADE20K/COCO-Stuff, 417.5 GFLOPs for Cityscapes) achieves 52.1\%, 83.8\%, and 47.7\% mIoU on these datasets respectively while maintaining competitive inference speed. 

To summarize, our contributions are threefold:
\begin{itemize}
    \item We introduce LAMNet, a novel encoder architecture featuring our LAM token mixer that synergistically combines local attention with state space models for efficient global context modeling and local detail encoding, achieving linear time complexity.
    \item We propose MMSCopE, a novel decoder module that operates on multi-scale feature maps that adaptively scale with the input resolution, surpassing previous approaches in both fine-grained detail preservation and omni-scale context learning.
    \item We demonstrate through comprehensive experiments that LAMSeg, powered by LAMNet and MMSCopE, establishes new state-of-the-art performance while maintaining competitive computational efficiency across multiple challenging semantic segmentation benchmarks.
\end{itemize}


==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/conclusion.tex <==


\section{Conclusion}
This work presents a new segmentation network with two novel components: LAMNet, a hierarchical encoder that synergistically integrates state space models with local attention, and MMSCopE, an efficient decoder module that leverages state space models for multi-scale context extraction.
LAMNet enables simultaneous modeling of fine-grained spatial details and global contextual information while MMSCopE adaptively scales with the input resolution while processing multi-scale features.
We conduct comprehensive evaluations across multiple benchmarks, which demonstrates that our approach achieves state-of-the-art performance in semantic segmentation.
%We hope that our network designs can advance research in high-resolution dense prediction tasks, particularly in applications requiring both local precision and global semantic understanding.

==> sec/experiments.tex <==
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\begin{table*}[t]
\centering
\scalebox{0.715}{
\begin{tabular}{lc|cc|cc|cc} 

\toprule
\multirow{2}{*}{Method}& \multirow{2}{*}{Params(M)} & \multicolumn{2}{c|}{ADE20K}  & \multicolumn{2}{c|}{Cityscapes} & \multicolumn{2}{c}{COCO-Stuff} \\

& & GFLOP & mIoU & GFLOP & mIoU & GFLOP & mIoU \\

\midrule
\midrule

Segformer-B0~\cite{xie2021segformer} & 3.8 & 8.4 & 37.4 & 125.5 & 76.2 & 8.4 & 35.6 \\
SegNeXt-T~\cite{guo2022segnext} & 4.3 & 7.7 & 41.1 & 61.6 & 78.9 & 7.7 & 38.7 \\
VWFormer-B0~\cite{yan2024vwaformer} & 3.7 & 5.8 & 38.9 & 112.4 & 77.2 & 5.8 & 36.2 \\
EDAFormer-T~\cite{yu2024edaformer} & 4.9 & 5.8 & 42.3 & 151.7 & 78.7 & 5.8 & 40.3 \\
CGRSeg-T$^{\dagger}$~\cite{ni2024cgrseg} & 9.4 & 4.8 & 42.5 & 65.5 & 78.3 & 4.8 & 40.4 \\
\rowcolor{ggray} LAMSeg-T & 5.1 & 4.6 & \textbf{43.3} & 59.7 & \textbf{80.0} & 4.6 & \textbf{40.8} \\

\midrule
% PSPNet~\cite{zhao2017pyramid} &  & &  &  &  & &  \\
% DeepLabV3+~\cite{} &  & &  &  &  & &  \\
Swin UperNet-T~\cite{liu2021swin} & 60.0 & 236.0 & 44.4 & - & - & - & - \\
ViT-CoMer-S~\cite{xia2024vit} & 61.4 & 296.1 & 46.5 & - & - & - & - \\
OCRNet~\cite{yuan2020ocrnet} & 70.5 & 164.8 & 45.6 & - & - & - & -\\
Segformer-B2~\cite{xie2021segformer} & 27.5  & 62.4 & 46.5 & 717.1 & 81.0 & 62.4 & 44.6 \\
MaskFormer~\cite{cheng2021maskformer} & 42.0 & 55.0 & 46.7 & - & - & - & - \\
Mask2Former~\cite{cheng2022masked2former} & 47.0 & 74.0 & 47.7 & - & - & - & - \\
SegNeXt-B~\cite{guo2022segnext} & 27.6 & 34.9 & 48.5 & 279.1 & 82.6 & 34.9 & 45.8 \\
FeedFormer-B2~\cite{shim2023feedformer} & 29.1 & 42.7 & 48.0 & 522.7 & 81.5 & -& - \\
VWFormer-B2~\cite{yan2024vwaformer} & 27.4 & 46.6 & 48.1 & 415.1 & 81.7 & 46.6 & 45.2 \\
EDAFormer-B~\cite{yu2024edaformer} & 29.4 & 32.1 & 49.0 & 605.9 & 81.6 & 32.1 & 45.9 \\
CGRSeg-L$^{\dagger}$~\cite{ni2024cgrseg} & 35.7 & 16.5 & 47.3 & 199.7 & 80.2 & 16.5 & 45.2 \\
\rowcolor{ggray} LAMSeg-S & 29.9 & 24.5 & \textbf{50.0} & 223.4 & \textbf{83.3} & 24.5 & \textbf{46.9}\\

\midrule
Swin UperNet-B~\cite{liu2021swin} & 121.0 & 261.0 & 48.1 & - & - & - & - \\
ViT-CoMer-B~\cite{xia2024vit} & 144.7 & 455.4 & 48.8 & - & - & - & - \\
Segformer-B3~\cite{xie2021segformer} & 47.3 & 79.0 & 49.4 & 962.9 & 81.7 & 79.0 & 45.5 \\
SegNeXt-L~\cite{guo2022segnext} & 48.9 & 70.0 & 51.0 & 577.5 & 83.2 & 70.0 & 46.5 \\
VWFormer-B3~\cite{yan2024vwaformer} & 47.3 & 63.3 & 50.3 & 637.1 & 82.4 & 63.3 & 46.8 \\
\rowcolor{ggray} LAMSeg-B & 53.9 & 52.9 & \textbf{52.1} & 417.5 & \textbf{83.8} & 52.9 & \textbf{47.7} \\
\bottomrule
\end{tabular}}
\caption{Comparison with state-of-the-art semantic segmentation models on ADE20K, Cityscapes, and COCO-Stuff-164K. GFLOPs is calculated at 512x512 resolution for ADE20K and COCO-Stuff, and at 2048x1024 resolution for Cityscapes.}
\label{exp_main_segmentation}
\vspace{-3mm}
\end{table*}


\section{Experiments}

\subsection{Setting}
\textbf{Datasets.}
% As in standard segmentation methods, the ImageNet-1K dataset~\cite{deng2009imagenet} was used to pre-train our LAMNet encoder. Then, we evaluate segmentation performance on three commonly-used datasets: ADE20K~\cite{zhou2017ade20k}, a challenging scene parsing benchmark containing 20,210 images annotated with 150 semantic categories; Cityscapes~\cite{cordts2016cityscapes}, an urban driving dataset of 5,000 high-resolution images with 19 semantic classes; and COCO-Stuff-164K~\cite{caesar2018cocostuff}, which comprise 164,000 images labeled across 172 semantic categories.
Following previous works \cite{xie2021segformer,guo2022segnext}, we firstly pre-train our LAMNet encoder on the ImageNet-1K dataset~\cite{deng2009imagenet}. Then, we evaluate the semantic segmentation performance on three commonly used datasets: ADE20K~\cite{zhou2017ade20k}, a challenging scene parsing benchmark consisting of 20,210 images annotated with 150 semantic categories; Cityscapes~\cite{cordts2016cityscapes}, an urban driving dataset comprising 5,000 high-resolution images with 19 semantic classes; and COCO-Stuff-164K~\cite{caesar2018cocostuff}, which contains 164,000 images labeled across 172 semantic categories.

\textbf{Implementation details.}
% ImageNet pre-training was conducted using the Timm~\cite{rw2019timm} library using hyperparameters and data augmentation settings of Swin Transformer~\cite{liu2021swin}. 
% Segmentation models were trained using the MMSegmentation~\cite{mmseg2020} library by using the pre-trained LAMNet encoder and a randomly initialized version of our decoder. 
% Following the training protocol in Segformer~\cite{xie2021segformer}, we employed standard data augmentation techniques including random horizontal flipping and random scaling (ratio 0.5-2.0). Dataset-specific random cropping was implemented with dimensions of 512×512 for ADE20K and COCO-Stuff, and 1024×1024 for Cityscapes. Training was performed using the AdamW optimizer for 160K iterations with batch sizes of 16 for ADE20K and COCO-Stuff, and 8 for Cityscapes.
% The evaluation metric for segmentation is mean intersection over union (mIoU) and we adopt the fvcore~\cite{fvcore} library for FLOP computation.
% Models were trained using 8 NVIDIA H100 GPUs.
We conducted ImageNet pre-training using the Timm library~\cite{rw2019timm} with hyperparameters and data augmentation settings identical to those of Swin Transformer~\cite{liu2021swin}. Regarding semantic segmentation, we trained all models using the MMSegmentation library~\cite{mmseg2020}, combining the pre-trained LAMNet encoder with a randomly initialized decoder.
Following the Segformer training protocol~\cite{xie2021segformer}, we employed standard data augmentation techniques, including random horizontal flipping and random scaling (ratio 0.5-2.0). We implemented dataset-specific random cropping with dimensions of 512×512 for ADE20K and COCO-Stuff, and 1024×1024 for Cityscapes. We trained the models using the AdamW optimizer for 160K iterations with batch sizes of 16 for ADE20K and COCO-Stuff, and 8 for Cityscapes.
We evaluated segmentation performance using mean intersection over union (mIoU) and computed FLOPs using the fvcore library~\cite{fvcore}.
All models were trained on 8 NVIDIA H100 GPUs.

\subsection{Comparison with state-of-the-art methods}
This section presents a comprehensive comparison of our proposed LAMSeg with state-of-the-art segmentation methods on three widely used datasets.
% aiming to showcase the effectiveness and efficiency LAMSeg. 

% scalability of

% ADE20K~\cite{zhou2017ade20k}, Cityscapes~\cite{cordts2016cityscapes}, and COCO-Stuff-164K~\cite{caesar2018cocostuff}. 

\textbf{Baselines.}
We compare our method with other strong competitors including EDAFormer~\cite{yu2024edaformer}, VWFormer~\cite{yan2024vwaformer} and CGRSeg~\cite{ni2024cgrseg}, Segformer~\cite{xie2021segformer}, and OCRNet~\cite{yuan2020ocrnet}.
% The feature encoders used for EDAFormer, VWFormer, and CGRSeg are EFT~\cite{yu2024edaformer}, MiT~\cite{xie2021segformer}, and Efficientformer-v2~\cite{li2022efficientformerv2} respectively.

Note that the Efficientformer-v2~\cite{li2022efficientformerv2} used in CGRSeg~\cite{ni2024cgrseg} significantly benefits from knowledge distillation from RegNetY-16GF~\cite{radosavovic2020designing} (83.6M parameters, 15.9 GFLOPs), providing a stronger encoder network compared to other methods. To ensure a fair comparison, we retrained Efficientformer-v2 on ImageNet-1K using the same training configurations as Swin. We report results for CGRSeg by fine-tuning this retrained encoder following official implementations.

% \footnote{https://github.com/nizhenliang/CGRSeg}. 

\textbf{Results.}
Table~\ref{exp_main_segmentation} shows the superior performance of LAMSeg across all three datasets: ADE20K, Cityscapes, and COCO-Stuff-164K. Among lightweight models, LAMSeg-T achieves the best performance, with 43.3\% mIoU on ADE20K, 80.0\% mIoU on Cityscapes, and 40.8\% mIoU on COCO-Stuff, while maintaining comparable computational costs for ADE20K and Cityscapes, respectively. 
Our LAMSeg-S model demonstrates more substantial improvements over existing methods, surpassing the recently updated EDAFormer-B~\cite{yu2024edaformer} by +1.0\% mIoU on both ADE20K and COCO-Stuff while reducing the computational cost by more than 20\% to 24.5 GFLOPs. On Cityscapes, LAMSeg-S achieves 83.3\% mIoU, surpassing EDAFormer-B by +1.7\%.
Moreover, LAMSeg-B surpasses previous best performing models by +1.1\% and +0.9\% mIoU on ADE20K and COCO-Stuff while reducing the computational cost by more than 15\% to 52.9 GFLOPs. On Cityscapes, LAMSeg-B improves mIoU by 0.6\% using 28\% less GFLOPs.
The consistent performance gains across different datasets and model scales validate the effectiveness of our proposed LAMSeg, which can simultaneously capture global context, local details, and multi-scale information through its LAMNet encoder and MMSCopE-based decoder. 
% Additionally, increasing parameters and GLFOPs for LAMSeg yield consistant and substantial improvements in the challenging ADE20K and COCO-Stuff benchmarks, demonstrating its scalability.


\textbf{Speed Analysis.}
We benchmark inference speed on Cityscapes~\cite{cordts2016cityscapes} using an NVIDIA L40S GPU, averaging Frames Per Second (FPS) over 128 steps with batch size 2.
As shown in Table~\ref{tab:latency_comparison}, LAMSeg-T achieves +1.2\% mIoU at approximately 3 times the speed of EDAFormer-T, highlighting an excellent balance between performance and speed.
% Similarly, LAMSeg-S surpasses VWFormer-B2 by 1.4\% mIoU while maintaining faster inference speed. These results demonstrate that our method strikes an excellent balance between performance and speed.

\begin{table}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
\scalebox{0.8}{
\begin{tabular}{lcccc}
\toprule
Model  & Params (M) & GFLOPs & FPS & mIoU \\
\midrule
\midrule
Segformer-B0~\cite{xie2021segformer} & 3.8 & 125.5 & 21.8& 76.2 \\
SegNext-T~\cite{guo2022segnext} & 4.3 & 61.6 & 25.8 & 78.9\\
VWFormer-B0~\cite{yan2024vwaformer} & 3.7 & 112.4 & 21.1 & 77.2\\
EDAFormer-T~\cite{yu2024edaformer} & 4.9 & 151.7 & 12.7 & 78.7 \\
CGRSeg-T~\cite{ni2024cgrseg}  & 9.3 & 65.5 & 27.6 & 78.3 \\
\rowcolor{ggray} LAMSeg-T & 5.1 & 59.7 & 35.5 & 80.0 \\
\midrule
Segformer-B2~\cite{xie2021segformer} & 27.5 & 717.1 & 10.2 & 81.0 \\
SegNext-B~\cite{guo2022segnext} & 27.6 & 279.1 & 14.1 & 82.6 \\
VWFormer-B2~\cite{yan2024vwaformer} & 27.4 & 415.1 & 9.87 & 81.7 \\
EDAFormer-B~\cite{yu2024edaformer} & 29.5 & 605.9 & 6.6 & 81.6 \\
CGRSeg-B~\cite{ni2024cgrseg} & 35.6 & 199.0 & 11.8 & 80.2 \\
\rowcolor{ggray} LAMSeg-S & 30.0 & 223.0 & 13.1 & 83.3 \\

\midrule
Segformer-B3~\cite{xie2021segformer} & 46.3 & 962.9 & 6.7 & 81.7 \\
SegNext-L~\cite{guo2022segnext} & 48.9 & 577.5 & 10.1 & 83.2 \\
VWFormer-B3~\cite{yan2024vwaformer} & 47.3 & 637.1 & 6.3 & 82.4 \\
\rowcolor{ggray} LAMSeg-B & 53.9 & 417.5 & 8.4 & 83.8 \\
\bottomrule
\end{tabular}}
\caption{Comparison of model complexity and inference speed on Cityscapes~\cite{cordts2016cityscapes} (2048×1024 resolution).}
\label{tab:latency_comparison}
\end{table}


% \begin{table}
% \setlength{\belowcaptionskip}{-0.2cm}
% \centering
% \scalebox{0.8}{
% \begin{tabular}{llccc}
% \toprule
% Model & Encoder & Params (M) & GFLOPs & FPS \\
% \midrule
% \midrule
% Segformer-B0~\cite{xie2021segformer} & MiT-B0 & 3.8 & 125.5 & 21.8 \\
% SegNext-T~\cite{guo2022segnext} & MSCAN-T & 4.3 & 61.6 & 25.8 \\
% EDAFormer-T~\cite{yu2024edaformer} & EFT-T & 4.9 & 151.7 & 12.7 \\
% CGRSeg-T~\cite{ni2024cgrseg} & EfficientFormerv2-S1 & 9.3 & 65.5 & 27.6 \\
% \rowcolor{ggray} Ours-T & LAMNet-T & 7.9 & 59.7 & 35.5 \\
% \midrule
% Segformer-B2~\cite{xie2021segformer} & MiT-B2 & 27.5 & 717.1 & 10.2 \\
% SegNext-B~\cite{guo2022segnext} & MSCAN-B & 27.6 & 279.1 & 14.1 \\
% EDAFormer-B~\cite{yu2024edaformer} & EFT-B & 29.5 & 605.9 & 6.6 \\
% CGRSeg-B~\cite{ni2024cgrseg} & EfficientFormerv2-L & 35.6 & 199.0 & 11.8 \\
% \rowcolor{ggray} Ours-S & LAMNet-S & 30.0 & 223.0 & 13.1 \\
% \bottomrule
% \end{tabular}}
% \caption{Comparison of model complexity and inference speed.}
% \label{tab:latency_comparison}
% \end{table}

% while Mamba has linear complexity, its GPU parallelization is not as profound as Transformers. 


\subsection{Comparison of different feature encoders}
In this section, we evaluate the classification performance of our proposed LAMNet on ImageNet-1K~\cite{deng2009imagenet}, comparing against two categories of architectures: state-of-the-art segmentation encoders (MiT~\cite{xie2021segformer}, MSCAN~\cite{xie2021segformer}, EFT~\cite{yu2024edaformer}) and representative vision backbones designed for dense prediction tasks (Swin Transformer~\cite{liu2021swin}, PVT~\cite{wang2021pyramid}, ConvNeXt~\cite{liu2022convnext}).
As demonstrated in Table~\ref{exp_encoder}, LAMNet variants consistently achieve superior classification accuracy in comparison to architectures of similar computational complexity. Specifically, LAMNet-S remarkably surpasses ConvNeXt-T and MSCAN-B by 1.9\% and 1.0\% in Top-1 accuracy, respectively. 
The larger LAMNet-B variant demonstrates similar improvements over Swin-S and MSCAN-L by 1.6\% and 0.9\%, respectively.
% While LAMNet-T shows marginally lower accuracy than MSCAN-T (0.66\% relative decrease), it achieves this with significantly reduced computational overhead, requiring 33\% fewer FLOPs. 
The promising performance across model variants demonstrates the benefits of integrating local attention with state space models to effectively capture both fine-grained details and global contextual information.

\begin{table}
\setlength{\belowcaptionskip}{-0.2cm}
\centering
\scalebox{0.8}{
\begin{tabular}{lccc} 

\toprule

Models  & Params (M) & GFLOPs & Acc \\
\midrule
\midrule
MiT-B0~\cite{xie2021segformer} & 3.8 &0.60 & 70.5 \\
EFT-T~\cite{yu2024edaformer} &3.7 &0.60 & 72.3 \\ %74.1 (lr2e-3)
MSCAN-T~\cite{guo2022segnext} & 4.2 & 0.89 & 75.9 \\
% EfficientFormerv2-S1~\cite{li2022efficientformerv2} & 6.1 &0.65 & 78.3 \\
\rowcolor{ggray} LAMNet-T & 3.5 & 0.65 & \textbf{76.2} \\
\midrule
% seg encoder
MiT-B2~\cite{xie2021segformer} & 24.2 & 4.0 & 81.6 \\
EFT-B~\cite{yu2024edaformer} & 26.4 & 4.2 & 82.4 \\
MSCAN-B~\cite{guo2022segnext} & 26.8 & 4.4 & 83.0 \\
% backbones
Swin-T~\cite{liu2021swin} & 28 & 4.5 & 81.2\\
PVT-S~\cite{wang2021pyramid} & 24.5 & 3.8 & 79.8 \\
ConvNeXt-T~\cite{liu2022convnext} & 28 & 4.5 & 82.1 \\
% EfficientFormerv2-l~\cite{li2022efficientformerv2} & 26.4 & 4.2 & 82.3 \\
\rowcolor{ggray} LAMNet-S & 25.5 & 4.1 & \textbf{84.0} \\
\midrule
% seg encoder
MiT-B3~\cite{xie2021segformer} & 45.2 & 6.9 & 83.1 \\
MSCAN-L~\cite{guo2022segnext} & 45.2 & 9.1 & 83.9 \\
% backbone
Swin-S~\cite{liu2021swin} & 50 & 8.7 & 83.2\\
PVT-M~\cite{wang2021pyramid} & 44.2 & 6.7 & 81.2 \\
ConvNeXt-S~\cite{liu2022convnext} & 50 & 8.7 & 83.1 \\
\rowcolor{ggray} LAMNet-B & 45.7 & 8.2 & \textbf{84.8} \\
\bottomrule
\end{tabular}}
\caption{Comparison of classification accuracy and computational complexity (FLOPs at \(224\times 224\) resolution) of encoder architectures on ImageNet-1K.}
\label{exp_encoder}
\end{table}

\subsection{Ablation studies on LAMSeg decoder}
To validate our architectural design choices, we conduct ablation studies on the ADE20K dataset~\cite{zhou2017ade20k}, examining both the overall effectiveness of our proposed decoder and the performance of individual components of the MMSCopE module. FLOPs and FPS are measured at \(512\times 512\) resolution. 
For a fair comparison, we ensure that different model variants have comparable computational complexity by adjusting the number of channels. Here, all ablations are conducted using the LAMSeg-S decoder.


% the channel sizes are adjusted to ensure all models have comparable parameters and GFLOPs.

\textbf{Comparision of decoders}.
% Since the representation capacity of the feature encoder significantly impacts segmentation performance~\cite{xie2021segformer,guo2022segnext,yu2024edaformer}, 
Table~\ref{tab:ablation_head_replace} shows a performance comparison of segmentation decoders. For a fair comparison, all models here share the same feature encoder, MSCAN-B~\cite{guo2022segnext}, and we adopt decoders from segmentation model variants~\cite{xie2021segformer,guo2022segnext,yan2024vwaformer,ni2024cgrseg,yu2024edaformer} with model size similar to that of LAMSeg-S, and adjusted UPerNet's channel dimension to match comparable GFLOPs. Notably, our proposed decoder demonstrates superior segmentation accuracy.

% We isolate decoder effectiveness by utilizing the same MSCAN-B~\cite{guo2022segnext} encoder for all segmentation decoders participating in this comparison. As shown in Table~\ref{tab:ablation_head_replace}, our proposed decoder achieves superior segmentation accuracy while maintaining competitive computational efficiency in terms of GFLOPs and inference speed.

\begin{table}[t]
\centering
\scalebox{0.77}{
\begin{tabular}{l c c c}
\toprule
Model & Params (M) & GFLOPs  & mIoU (\%) \\
\midrule
UPerNet~\cite{xiao2018unified} & 27.2 & 30.4  & 46.1 \\
MLP Decoder~\cite{xie2021segformer} & 26.5 & 28.5 & 47.0 \\
Ham Decoder~\cite{guo2022segnext} & 27.7 & 34.9 & 48.5 \\
VWFormer Decoder~\cite{yan2024vwaformer} & 26.9 & 29.5 & 46.7 \\
CGRHead~\cite{ni2024cgrseg} & 47.2 & 29.9 & 48.2 \\
EDAFormer Decoder~\cite{yu2024edaformer} & 30.9 & 31.6 & 48.3 \\
\rowcolor{ggray}LAMSeg-S Decoder & 30.6 & 29.9  & 48.9 \\
\bottomrule
\end{tabular}}
\caption{Comparison of complexity and accuracy of segmentation decoders. FLOPS and FPS are measured at \(512\times 512\) resolution.\vspace{-6mm}} 
\label{tab:ablation_head_replace}
\end{table}


\textbf{Ablation studies on the MMSCopE module.}
Here, we investigate the design choices of the MMSCopE module and feature fusion strategy in our decoder. 
Table~\ref{tab:ablation_within_head_mmscope} presents the impact of various components within the MMSCopE module: (1) Switching to independently scanning each feature map instead of our proposed simultaneous scanning strategy significantly reduces FPS from 129 to 67; (2) The inclusion of multi-scale features yields consistent performance gains. Specifically, removing the feature map at 16x16, 32x32, or 64x64 resolution inside the MMSCopE module results in sub-optimal mIoU, with the removal of the 64x64 feature map resulting in the largest performance drop of 0.6\%. Additionally, using the 64x64 feature map alone without pixel unshuffling and compression leads to a 0.3\% decline.
(3) Channel compression before SS2D proves beneficial, as its removal reduces mIoU by 0.3\%. Alternative channel scaling configuration (1C, 2C, 4C) for the three feature scales yields suboptimal results; (4) The FFN following SS2D provides a marginal benefit of 0.2\%.

\textbf{Effect of feature fusion in the decoder.}
Table~\ref{tab:ablation_within_head_decoder} illustrates the importance of our feature fusion approach (Figure~\ref{method_model}(c)). Direct prediction from multi-scale context feature \(F'\) results in significant performance degradation (-0.7\%). While incorporating the feature map \(F\) improves performance to 49.7\%, our fusion strategy with stage-specific features \(F'_2\), \(F_{up3}\) \(F_{up4}\) achieves the optimal performance of 50\% mIoU.
Removal of average-pooled features and not adding \(F'\) to stage specific features reduces effectiveness. For a fair comparison, average-pooled features are included in experiments without stage-specific features.

\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{lccccc}
\toprule
Model Variant & Params (M) & GFLOPs & FPS & mIoU \\
\midrule
\midrule
LAMSeg-S & 29.9 & 24.6 & 129 & 50.0 \\
\midrule
\multicolumn{5}{l}{\textit{Scan Strategy}} \\
Independent scans & 28.4 & 25.0 & 67 & 49.9(-0.1) \\
\midrule
\multicolumn{5}{l}{\textit{Multi-scale feature}} \\
w/o 16×16 & 29.4 & 24.4 & 130 & 49.8 (-0.2) \\
w/o 32×32 & 29.0 & 24.3 & 132 & 49.6 (-0.4) \\
w/o 64×64 & 28.8 & 24.1 & 131 & 49.4 (-0.6) \\
64×64 only & 26.2 & 23.6 & 137 & 49.7 (-0.3) \\
\midrule
\multicolumn{5}{l}{\textit{Compression}} \\
w/o compression & 30.8 & 25.9 & 102 & 49.7 (-0.3) \\
Channels 1C:2C:4C & 31.2 & 25.3 & 124 & 49.8 (-0.2) \\
\midrule
\multicolumn{5}{l}{\textit{Architecture Components}} \\
w/o FFN & 28.7 & 24.2 & 130 & 49.8 (-0.2) \\
\bottomrule
\end{tabular}}
\caption{Ablation studies on the MMSCopE module in LAMSeg decoder.\vspace{-2mm}}
\label{tab:ablation_within_head_mmscope}
\end{table}


\begin{table}[t]
\centering
\scalebox{0.8}{
\begin{tabular}{lccc}
\toprule
Input to classifier & Params (M) & GFLOPs  & mIoU \\
\midrule
\midrule
LAMSeg-S & 29.9 & 24.6  & 50.0 \\
\midrule
\multicolumn{4}{l}{\textit{w/o stage-specific features}} \\
Concat (\(F\),\(F'\)) & 30.0 & 24.0  & 49.7 (-0.3) \\
\(F + F'\) & 29.7 & 23.9  & 49.5 (-0.5) \\
\(F'\) & 29.7 & 23.7  & 49.3 (-0.7) \\

\midrule
\multicolumn{4}{l}{\textit{w stage-specific features}} \\
w/o avg pool & 29.8 & 24.3  & 49.7 (-0.3) \\
w/o addition & 29.9 & 24.4  & 49.9 (-0.1) \\

\bottomrule
\end{tabular}}
\caption{Effect of fusion strategies in the LAMSeg decoder.\vspace{-3mm}}
\label{tab:ablation_within_head_decoder}
\end{table}

\subsection{Ablation studies on LAMNet encoder}
This section presents a systematic investigation of LAMNet's architectural design choices through experiments on both ImageNet-1K~\cite{deng2009imagenet} and ADE20K~\cite{zhou2017ade20k} using the LAMNet-S model. The token mixer MAMixer in LAMNet stacks Neighborhood Attention (Natten)~\cite{hassani2023neighborhoodAttn} and 2D-Selective-Scan (SS2D) in series with a residual connection added to the SS2D module to merge global and local contexts. And global attention instead of SS2D is employed in Stage 4 blocks.

To validate these architectural decisions, we conduct comprehensive ablation studies examining: (1) comparative performance against alternative token mixers, (2) design choices of MAMixer, and (3) the impact of individual components within the token mixer. In all experiments, including token mixer replacements, we maintain consistent model complexity by adjusting channel dimensions to achieve comparable parameter counts and computational costs. Table~\ref{tab:ablation_backbone} presents our findings.

\textbf{Alternative token mixers.}
We evaluate the effectiveness of MAMixer by replacing it with recent token mixers (MaxViT~\cite{tu2022maxvit}, ACMix~\cite{pan2022acmix}, PVT~\cite{wang2021pyramid}, and BiFormer~\cite{zhu2023biformer}). Note that we implement MaxViT's Block-SA and Grid-SA modules in series to serve as a token mixer. As shown in Table~\ref{tab:ablation_backbone}, our MAMixer achieves consistent and substantial improvements across both classification and segmentation tasks while maintaining competitive computational costs. The performance gains stem from the complementary nature between Natten, which models fine-grained local features and SS2D, which efficiently models global contexts.

\textbf{Alternative MAMixer designs.} We explore alternative methods to integrate SS2D and Natten together in MAMixer. Results indicate that parallel arrangement of Natten and SS2D and removing the residual connections for SS2D lead to substantial performance drops in both classification accuracy and segmentation mIoU.

\textbf{SS2D and Natten.}
We analyze the two key components of MAMixer through systematic ablations. When SS2D is replaced with alternative global attention mechanisms, performance consistently decreases: SRA~\cite{wang2021pyramid} (-0.3\% accuracy, -0.4\% mIoU) and Linear Attention~\cite{katharopoulos2020transformers} (-0.4\% accuracy, -1.1\% mIoU). Likewise, replacing Natten with either convolutions (-0.9\% accuracy, -1.4\% mIoU) or Swin~\cite{liu2021swin} (-0.5\% accuracy, -0.8\% mIoU) leads to significant performance degradation, demonstrating the effectiveness of our component choices.



\begin{table}[t]
\centering
\scalebox{0.73}{
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{Model Variant} & Params & \multirow{2}{*}{GFLOPs}  & \multirow{2}{*}{Acc} & \multirow{2}{*}{mIoU} \\
 & (M) & & & \\
\midrule
\midrule
LAMNet-S & 25.5 & 4.0  & 84.0 & 50.0 \\
\midrule
\multicolumn{5}{l}{\textit{Replace MAMixer}} \\
MaxViT~\cite{tu2022maxvit} & 24.6 & 3.9  & 83.5 (-0.5) & 46.9 (-3.1)\\
ACMix~\cite{pan2022acmix} & 24.9 & 3.8  & 83.1 (-0.9) & 48.0 (-2.0) \\
PVT~\cite{wang2021pyramid} & 29.5 & 3.7  & 82.8 (-1.2) & 48.6 (-1.4) \\
BiFormer~\cite{zhu2023biformer} & 25.2 & 4.1  & 82.9 (-1.1) & 48.3 (-1.7) \\

\midrule
\multicolumn{5}{l}{\textit{MAMixer Design}} \\
Parallel Natten and SS2D & 25.5 & 4.1  & 83.8 (-0.2) & 47.4 (-2.6) \\
w/o SS2D residual & 26.1 & 4.1  & 83.7 (-0.3) & 49.3 (-0.7) \\
Stage 4 Attn → SS2D & 30.0 & 4.1  & 83.7 (-0.3) & 49.4 (-0.6) \\

\midrule
\multicolumn{5}{l}{\textit{SS2D within MAMixer}} \\
Replace SS2D w SRA~\cite{wang2021pyramid} & 26.0 & 4.2  & 83.7 (-0.3) & 49.6 (-0.4) \\
Replace SS2D w L-Attn~\cite{katharopoulos2020transformers} & 27.6 & 4.1  & 83.6 (-0.4) & 48.9 (-1.1) \\
Remove SS2D & 25.0 & 3.9  & 83.6 (-0.4) & 46.5 (-3.5) \\
\midrule
\multicolumn{5}{l}{\textit{Natten within MAMixer}} \\
Replace Natten w Conv & 25.8 & 3.8  & 83.1 (-0.9) & 48.6 (-1.4)\\
Replace Natten w Swin~\cite{liu2021swin} & 30.0 & 4.1  & 83.5 (-0.5) & 49.2 (-0.8) \\
Remove Natten~\cite{hassani2023neighborhoodAttn} & 24.9 & 4.1  & 83.6 (-0.4) & 48.9 (-1.1) \\

\bottomrule
\end{tabular}}
\caption{Ablation studies and comparison of token mixers for LAMSeg encoder. Parameters, FLOPs and FPS are calculated or measured at \(224\times 224\) resolution using the encoder.\vspace{-3mm}}
\label{tab:ablation_backbone}
\end{table}


==> sec/method.tex <==
\section{Method}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.9\textwidth]{sec/Figures/encoder.pdf}
% \caption{Network architecture of LAMNet. \textit{Left:} Architecture of LAMNet. \textit{Right:} The Local Attention Mamba module.}
% \label{method_fig_encoder}
% \end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=0.98\textwidth]{sec/Figures/model.pdf}
\caption{Overall Architecture of LAMSeg. (a) Hierarchical encoder LAMNet. (b) Mamba-Attention Mixer (MAMixer) for modeling global contexts and local details with linear complexity. (c) The decoder of LAMSeg. (d) The MMSCopE module, which leverages Mamba-based 2D-selective-scan (SS2D) to extract contexts at multiple scales.}
\label{method_model}
\end{figure*}

\subsection{Overall Architecture}
As shown in Figure~\ref{method_model}, our proposed ModelName consists of a pair of newly designed feature encoder and decoder. Specifically, we propose a novel hybrid feature encoder based on core mechanisms from both Transformer and Mamba (LAMNet), and a simple yet effective Mamba-based Multi-Scale Context Extraction Decoder (MMSCopE) as the decoder. LAMNet has a hierarchical architecture that integrates the 2D-Selective-Scan Block (SS2D in VMamba)~\cite{liu2024vmamba} with Neighborhood Attention (Natten)~\cite{hassani2023neighborhoodAttn} within the token mixer, enabling comprehensive feature learning at both global and local scales across all layers while maintaining linear computational complexity. Meanwhile, MMSCoPE dynamically and adaptively extracts multi-scale semantic information by processing feature maps at varying levels of granularity using SS2D~\cite{liu2024vmamba}, with the scales adaptively adjusted according to the input resolution. Collectively, LAMNet injects robust global contexts and local details into a feature pyramid, where feature maps are progressively downsampled and transformed to produce omni-scale features at different pyramid levels. This feature pyramid is then fed into MMSCoPE, where features are further aggregated spatially as well as across scales, resulting in comprehensive multi-scale representations that can be used for dense prediction.

% In this section, we present a novel framework based on Mamba~\cite{gu2023mamba} for effective modeling of global context, local details, and multi-scale information. The linear complexity of Mamba facilitates efficient learning of global context and enables scalability to high spatial resolutions commonly found in segmentation datasets such as Cityscapes~\cite{cordts2016cityscapes} with \(2048\times 1024\) pixels. In contrast, conventional operators such as Convolutional Neural Networks (CNNs) and Transformers face significant challenges due to high resolution. CNNs struggle to model global contextual relationships due to their localized receptive fields~\cite{linsley2018learning, wang2021pyramid}, while Transformers face computational constraints arising from quadratic complexity with respect to sequence length.
% Although recent advancements in linear-complexity Transformers attempt to address these limitations, they often compromise either global receptive field capacity (e.g., windowed attention approaches~\cite{beltagy2020longformer, liu2021swin}) or overall performance (e.g., linear attention mechanisms~\cite{katharopoulos2020transformers}).

% Based on Mamba, we propose a framework comprising two complementary components: LAMNet, a feature encoder that integrates Mamba with local attention, and MMSCoPE (Mamba-based Multi-Scale Context Extraction) decoder. 
% LAMNet integrates Mamba with local attention within the token mixer, enabling comprehensive context modeling at both local and global scales while maintaining linear computational complexity.  
% MMSCoPE dynamically extracts semantic information across multiple spatial scales, adaptively adjusting its processing according to input resolution. 
% % MMSCoPE dynamically extracts semantic information across multiple spatial scales by processing feature maps at varying levels of granularity using Mamba operations, with the scales adaptively adjusted according to the input resolution. 
% Collectively, LAMNet ensures robust feature extraction with both global and local context, while MMSCoPE efficiently extracts multi-scale representation.


\subsection{Feature encoder}
\textbf{Overview.}
As shown in Figure~\ref{method_model}, our LAMNet encoder is a standard four-stage network~\cite{liu2021swin,liu2022convnext}, where each stage begins with a strided 3$\times$3 convolution for spatial reduction, followed by a series of LAMNet Blocks. Each LAMNet Block includes pre-layer normalization, a novel MAMixer, and a feedforward network (FFN)~\cite{liu2021swin, hassani2023neighborhoodAttn}.
Our proposed MAMixer represents the first integration of local self-attention (Natten~\cite{hassani2023neighborhoodAttn}) and state space models (SS2D~\cite{liu2024vmamba}) for semantic segmentation, capturing local details and global contexts simultaneously with linear time complexity. Ablation studies (Table~\ref{tab:ablation_backbone}) confirm the necessity of both components.
%- removing either significantly reduces segmentation performance, even when models have similar complexity in terms of parameters and GFLOPs.

% A residual connection is added to the Mamba module such that the global context extracted by Vision Mamba is integrated with the fine-grained local details captured by local attention.
% Our design enhances local precision and global semantic understanding, effectively mitigating errors at object boundaries and inter-class inconsistency for large objects.

\textbf{MAMixer.}
Long-range dependency modeling is crucial for semantic segmentation as they enable comprehensive context learning and scene understanding, as demonstrated by the success of Transformer-based semantic segmentation models~\cite{zheng2021SETR,ranftl2021vision,xie2021segformer,lu2023content,yu2024edaformer}.
To efficiently learn global contexts across all network layers, we leverage the SS2D block in VMamba~\cite{liu2024vmamba}. This variant of Mamba adopts four distinct and complementary scanning paths, enabling each token to integrate information from all other tokens in four different directions.

However, while Mamba achieves linear time complexity by compressing the global context of each channel into a fixed-dimensional hidden state~\cite{gu2023mamba}, this compression inherently leads to information loss, in particular, loss of fine-grained local spatial details, that are crucial in segmentation to accurately localize region boundaries. To this end, we utilize Neighborhood Attention (Natten)~\cite{hassani2023neighborhoodAttn}, where a sliding-window attention mechanism localizes every pixel's attention span to its immediate neighborhood. This approach retains translational equivalence, effectively captures local dependencies, and has linear time complexity. In practice, we serially stack Natten and SS2D, and a shortcut around SS2D is employed to merge local and global information. The merged output is then fed into a 1$\times$1 convolution layer for further global-local feature fusion.


\begin{table}[t]
\centering
\scalebox{0.75}{
\begin{tabular}{ccccc}
\toprule
LAMNet & Channels & Blocks & Params (M) & GFLOPs \\
\midrule
\midrule
Tiny & [32, 64, 144, 192] & [2, 2, 4, 2] & 3.5 & 0.65 \\
Small & [64, 144, 288, 512] & [2, 2, 10, 4] & 25.5 & 4.05 \\
Base & [72, 144, 320, 576] & [2, 2, 22, 4] & 45.7 & 8.2 \\
\bottomrule
\end{tabular}}
\caption{Configurations of the three LAMNet variants. FLOPs were measured at the \(224 \times 224\) resolution.}
\label{method_model_config}
\end{table}


\textbf{Network architecture.}
Our LAMNet produces a feature pyramid. The spatial resolution of \(F_i\) is \(\frac{H}{2^{1+i}} \times \frac{W}{2^{1+i}} \), where \(H\) and \(W\) are the height and width of the input image, respectively. We design three LAMNet variants with different model sizes, each with computational complexity comparable to some existing semantic segmentation encoders~\cite{xie2021segformer,guo2022segnext,yu2024edaformer}. 
As the feature map resolution at Stage 4 is (\(\frac{H}{32} \times \frac{W}{32}\)), global self-attention~\cite{vaswani2017attention} becomes computationally feasible. Therefore we replace SS2D with this more powerful global context modeling mechanism.
The configurations of these models are presented in Table~\ref{method_model_config}.


\subsection{Feature Decoder}
\textbf{Overview.} As shown in Figure~\ref{method_model}, our proposed decoder first aggregates features at various levels of abstraction (from low-level \(F_2\) to high-level \(F_4\)) to obtain a feature map \(F\) of size \(\frac{H}{8} \times \frac{W}{8} \), as in prior works~\cite{xie2021segformer,yan2024vwaformer}.
Specifically, each feature map \(F_i\) is projected to a lower dimension using a \(1\times 1\) convolution followed by batch normalization and ReLU, collectively denoted as `Conv' in Figure~\ref{method_model}. 
Subsequently, \(F_3\) and \(F_4\) are upsampled using bilinear interpolation to match the spatial dimensions of \(F_2\). 
The upsampled features \(F_{up3}\) and \(F_{up4}\) are concatenated together with \(F_2\) and passed through a Conv layer for channel dimension reduction, resulting in \(F\) with size \(\frac{H}{8} \times \frac{W}{8} \times C\), where \(C\) is the number of channels. 
The feature map \(F\) is then processed by our proposed MMSCopE module to extract rich multi-scale context features, producing a new feature map \(F'\).
We then add the feature map \(F'\) to \(F_{2}\), \(F_{up3}\), and \(F_{up4}\) to enrich their multi-scale contexts. The final prediction pathway concatenates \(F'\) with these context-enhanced features and the global pooling result on \(F_{up4}\), passes the combined features through a two-layer MLP, and the result is upsampled to the input resolution.


\textbf{Mamba-based multi-scale context extraction.}
% Current state-of-the-art segmentation decoders cannot effectively utilize local detail, global context, and multi-scale context simultaneously. 
% For instance, multiple pre-defined window sizes in VWFormer~\cite{yan2024vwaformer} can effectively collect multi-scale context from different scales. However, as the input resolution increases, these predefined windows cover only limited regions of the feature map, reducing its capacity to capture global context of the feature map.
% On the other hand, EDAFormer~\cite{yu2024edaformer} uses spatial reduction attention~\cite{wang2021pyramid}, sacrificing fine-grained spatial details by reducing the resolution of keys and values.
% To effectively utilize multi-scale, global, and local context simultaneously, we propose the Mamba-based Multi-Scale Context Extraction (MMSCoPE) module, which effectively extracts context at different scales from the feature map, covers the full feature map regardless of the input resolution, and maintains the original spatial resolution of feature maps during modeling.

To effectively extract contexts at different scales, we propose a Mamba-based Multi-Scale Context Extraction (MMSCoPE) module. As shown in Figure~\ref{method_model}, we apply strided convolutions to downsample the feature map \(F\), generating \(F_{s2}\) and \(F_{s4}\) with a resolution equal to 1/2 and 1/4 of that of \(F\), respectively. 
The motivation behind this is to obtain larger-scale representations through two derived feature maps: \(F_{s2}\), which aggregates features from \(3\times 3\) neighborhoods using a convolution with stride 2, and \(F_{s4}\), which aggregates features from \(5\times 5\) neighborhoods with stride 4.
% The spatial resolution of the feature maps is relative to the input resolution and the largest map \(F\) is processed globally independent of the input resolution, which cannot be achieved by VWFormer~\cite{yan2024vwaformer}.
Then, motivated by the observation that Mamba scans each channel independently, we use a single Mamba scan to simultaneously extract contexts from the three feature maps \(F\), \(F_{s2}\), and \(F_{s4}\).
The main idea is to concatenate these feature maps along the channel dimension and perform a single Mamba scan, which is more efficient on the GPU than processing each feature map separately.
However, the spatial dimensions of these feature maps are not consistent, which prevents direct concatenation. To resolve this, we employ lossless downsampling via the \emph{Pixel Unshuffle}~\cite{shi2016real} operation to reduce the spatial dimensions of \(F\) and \(F_{s2}\) to match that of \(F_{s4}\), which is \(\frac{H}{32} \times \frac{W}{32}\). 
Specifically, this operation rearranges non-overlapping 4×4 patches from \(F\) and 2×2 patches from \(F_{s2}\) into their respective channel dimension, increasing the channel depth by a factor of 16 and 4 respectively, while preserving complete spatial information. 
The transformed feature maps retain information at their original scales.
To reduce computational costs, we project each feature map to a fixed channel dimension \(C\) through \(1\times 1\) convolutions. This step assigns equal importance to the context information from each scale.
Then we concatenate the projected feature maps along the channel dimension, and pass the combined feature map to SS2D~\cite{liu2024vmamba} to achieve multi-scale context extraction in a single scan.
The resulting feature map is of size \(\frac{H}{8} \times \frac{W}{8} \times 3C\), where the three segments along the channel dimension correspond to earlier feature maps at three distinct scales (\(F\), \(F_{s2}\), and \(F_{s4}\)).
To facilitate context mixing across scales, we append a \(1\times 1\) convolution layer after the SS2D scan.
Finally, we use bilinear interpolation to upsample the mixed features to 1/8 input resolution, and project the channel dimension down to \(C\) using another \(1\times 1\) convolution. This yields the new feature map \(F'\) with mixed multi-scale contexts.

\textbf{Multi-scale fusion.}
Instead of directly using the feature map \(F'\) to predict pixel labels, we further exploit stage-specific representations from the encoder by adding \(F'\) to \(F_{2}\), \(F_{up3}\), and \(F_{up4}\). This effectively injects multi-scale contexts into stage-specific feature maps, which inherits information from various levels of abstraction.
Next, we concatenate the context-enhanced feature maps from each stage, the multi-scale context feature \(F'\), and the global average pooling result on \(F_{up4}\).
%This concatenation assembles information from various levels of abstraction, as well as multi-scale context and global semantics into a unified representation.
% as well as capturing fine-grained local details, regional context, and global semantics into a unified representation.
For pixel-wise label prediction, the diverse concatenated features are fused through a two-layer MLP, and further bilinearly interpolated to restore the original input resolution.


==> sec/related_work.tex <==
\section{Related work}

\textbf{Segmentation encoders.}
% Semantic segmentation extends image classification to the pixel level and is a fundamental computer vision task. 
Prior research in semantic segmentation architectures typically comprises two key components: an encoder for feature extraction from input images and a decoder for multi-scale context learning and pixel-wise classification. While conventional approaches often adapt popular classification networks such as ResNet~\cite{he2016deep}, ConvNeXt~\cite{liu2022convnext}, PVT~\cite{wang2021pyramid}, and Swin-Transformer~\cite{liu2021swin} as encoders, improvements in classification performance do not necessarily translate to enhanced segmentation capabilities~\cite{he2019bag}, primarily due to the requirement for fine-grained spatial information in segmentation tasks.
This observation has motivated the development of specialized segmentation-oriented encoders~\cite{zheng2021SETR,ranftl2021vision,xie2021segformer,guo2022segnext,yang2022lite,tang2023dynamic,yu2024edaformer,xia2024vit}. 
In this paper, we introduce a novel segmentation encoder that integrates local attention with Mamba. Different from previous works, our design enables the simultaneous modeling of fine-grained details and global contexts while maintaining linear time complexity.

\textbf{Segmentation decoders.}
Multi-scale feature learning plays a fundamental role in semantic segmentation, leading to numerous innovations in decoder architectures. Seminal works established various approaches to multi-scale feature aggregation, including the adaptive pooling strategy of PSPNet~\cite{zhao2017pyramid}, atrous convolutions in the DeepLab series~\cite{chen2017deeplab,Chen2017RethinkingAC, chen2018encoder}, and feature pyramid network (FPN) based decoders such as UPerNet~\cite{xiao2018unified} and Semantic FPN~\cite{kirillov2019panoptic}.
Contemporary architectures have advanced both efficiency and performance through diverse approaches to multi-scale feature fusion, including MLP-based methods (Segformer~\cite{xie2021segformer}), Matrix decomposition modules (SegNext~\cite{geng2021hamburger, guo2022segnext}), Transformers (FeedFormer~\cite{shim2023feedformer}, VWFormer~\cite{yan2024vwaformer}), and convolutions (CGRSeg~\cite{ni2024cgrseg}). 
An approach relevant to ours is VWFormer~\cite{yan2024vwaformer}, which employs cross-attention between local windows and multiple larger windows with predefined scales to capture multi-scale contexts. However, its reliance on fixed window scales limits its global context modeling capability: as the input resolution increases, the predefined windows fail to maintain complete feature map coverage. 
In contrast, our proposed decoder adaptively extracts context features at different scales while maintaining full feature map coverage regardless of the input resolution.

\textbf{Vision Mamba.} Dynamic state space models represented by Mamba~\cite{gu2023mamba,dao2024mamba2} have demonstrated promising performance in sequence modeling. Mamba combines structured state space models~\cite{gu2021efficiently,gu2021combining,gu2023mamba,smith2022simplified} with selective scanning, enabling global context modeling with dynamic weights and linear time complexity.
These favorable properties have led to promising results on vision tasks. For example, VMamba~\cite{liu2024vmamba}, PlainMamba~\cite{yang2024plainmamba}, and ViM~\cite{zhu2024vim} are Mamba-based vision backbone networks. 
Other works have explored Mamba for medical imaging~\cite{liu2024swin,ruan2024vm,xing2024segmamba}, 3D point clouds~\cite{zhang2024point,liu2024point,liang2024pointmamba}, and image/video generation~\cite{fei2024DiS,hu2024zigma,oshima2024ssm,teng2024dim,fu2024lamamba,fei2024dimba}.
In this paper, we leverage Mamba to learn global contexts in the encoder and multi-scale contexts in the decoder for segmentation.

